LifeBench: A Benchmark for Long-Horizon Multi-Source Memory

Long-term memory is fundamental for personalized agents capable of accumulating knowledge, reasoning over user experiences, and adapting across time. However, existing memory benchmarks primarily target declarative memory, specifically semantic and episodic types, where all information is explicitly presented in dialogues. In contrast, real-world actions are also governed by non-declarative memory, including habitual and procedural types, and need to be inferred from diverse digital traces. To bridge this gap, we introduce Lifebench, which features densely connected, long-horizon event simulation. It pushes AI agents beyond simple recall, requiring the integration of declarative and non-declarative memory reasoning across diverse and temporally extended contexts. Building such a benchmark presents two key challenges: ensuring data quality and scalability. We maintain data quality by employing real-world priors, including anonymized social surveys, map APIs, and holiday-integrated calendars, thus enforcing fidelity, diversity and behavioral rationality within the dataset. Towards scalability, we draw inspiration from cognitive science and structure events according to their partonomic hierarchy; enabling efficient parallel generation while maintaining global coherence. Performance results show that top-tier, state-of-the-art memory systems reach just 55.2\% accuracy, highlighting the inherent difficulty of long-horizon retrieval and multi-source integration within our proposed benchmark. The dataset and data synthesis code are available at https://github.com/1754955896/LifeBench.

==> Archive/acl/sections-2025dec/intro.tex <==
Daily life trajectory data from end-user devices is characterized by long temporal spans, heterogeneous data types, and complex multimodal patterns. However, the lack of mechanisms to align synthetic data with real-world behavior often results in deviations in factual consistency and semantic reliability. Existing generation methods typically produce simplified, templated, or averaged behavioral patterns that fail to capture the richness and variability of human activities. In practice, personal mobile data are collected over extended periods---often one to two years corresponding to a device's lifecycle---which further underscores the challenge of producing high-fidelity synthetic data that reflects realistic, long-term usage dynamics. To support downstream analysis, modeling, and evaluation, synthetic data must therefore achieve realism, temporal and semantic consistency, and sufficient behavioral diversity.

In addition to the inherent challenges of generating realistic end-user behavioral data, the evaluation of synthetic human-centric data remains underdeveloped. Current practice largely relies on manual inspection or ad-hoc expert judgement, which is labor-intensive, subjective, and difficult to reproduce at scale. The absence of systematic, quantitative, and domain-aligned evaluation metrics makes it challenging to rigorously assess the factual correctness, behavioral coherence, and semantic reliability of generated data. Moreover, without standardized benchmarks or reference baselines, it is difficult to compare different generation methods or quantify improvements. This lack of a robust evaluation framework ultimately limits the reliability and practical deployment of synthetic data in downstream applications.


==> Archive/acl/sections-2025dec/rw_data_synthetic.tex <==
\subsection{Personal 
Knowledge Graph: Applications}

Personal Knowledge Graphs offer multiple applications
1. recommendation
2. phone operation optimization
3. QA and agent memory: timelineQA, lifelogQA, locomo, mem-pal

\textbf{Digital Individual} 
The idea of building a knowledge base that can record all-dimensional information of an individual's life can be traced back to the concept of the Memex system (\citealp{bush1945we}). The MyLifeBits system (\citealp{gemmell2006mylifebits}) realized this idea using existing technologies from the late 1990s. Musto (\citealp{musto2018framework}) took the lead in proposing an integrated user modeling framework that fuses heterogeneous digital footprints,which integrating multi-source data of users from social networks and personal devices, and portrays users from 8 dimensions. Cyber-I models(\citealp{guo2018user}) conducted research on the evolution and construction of user models, integrating the Affective-Behavioral-Cognitive dimensions.
The "Lifelog Search Challenge (LSC)" explore the concept of Lifelogs. Lifelogs are systematic descriptions of events experienced by individuals, generated by fusing data from various digital services, such as online photos, map navigation, shopping records, and content streaming services. LSC focuses on lifelog retrieval and life event recognition. Although works like TimelineQA(\citealp{tan2023timelineqa}) and OpenLifelogQA(\citealp{tran2025openlifelogqa}) have designed QA benchmarks for lifelogs, these studies only focus on event memory, and do not involve how to extract events from fragmented, unstructured distributed device information.

\subsection{Personal Knowledge Graph: Data Synthetic}



\textbf{Personal Data Synthesis}
Personal-related data typically involves issues such as high costs and significant privacy risks, resulting in a scarcity of public datasets, Large Language Models (LLMs) demonstrate exceptional capabilities in reasoning, planning, and few-shot learning, while being able to learn from training data and simulate diverse human behaviors, and have been applied in political science, economics, and other social science research fields, in recent years, several studies have proposed methods for simulating human-related data using LLMs: TrajLLM(\citealp{ju2025trajllm}) utilizes LLMs to simulate human mobility trajectories, it not only integrates the ability of LLMs to generate coherent and interpretable human activities but also incorporates an innovative physical model for location mapping, addressing issues such as high costs and privacy concerns associated with traditional models; GATSim(\citealp{liu2025gatsim}) constructs generative agents with diverse socioeconomic attributes, personalized lifestyles, and dynamically evolving preferences, it performs travel decision-making through a psychology-compliant memory system, tool-using capabilities, and lifelong learning mechanisms, suitable for urban mobility simulation scenarios; LoCoMo(\citealp{maharana2024evaluating}) infers coherent event sequences of specific individuals through LLMs, using them as synthetic corpora for long-term dialogue data and question-answering (QA) data; TimelineQA(\citealp{tan2023timelineqa}) synthesizes personal event data based on user profiles, combining predefined rules and probabilistic graph models; APPGen(\citealp{huang2025appgen}) generates mobile application usage behavior data based on user movement trajectories, incorporating situational information and historical interaction data, it uses diffusion models to simulate the inherent uncertainty of application usage behaviors.

\subsection{Data Synthetic Evaluation}
\textbf{Logical Consistency} Due to the problems of hallucinations and insufficient logical capabilities of large language models, the content generated by large language models often lacks authenticity or contains logical problems. Scholars often use a variety of methods to solve this problem, including retrieval and inspection. For example, RIGOR (\citealp{DBLP:journals/corr/abs-2506-01232}) and CRP-RAG (\citealp{electronics14010047}) use retrieval to enhance the authenticity and logic of model generation from the perspective of text generation. Methods ExKLoP (\citealp{DBLP:journals/corr/abs-2502-12275}), and FlawedFictionsMaker (\citealp{DBLP:journals/corr/abs-2506-01232}) help diagnose and analyze generated content by using large models to analyze hallucinations and find logical problems. Both of these methods can solve the problem to a certain extent, but in the final analysis, they only use the ability of large language models to rely on context rather than the principle of generating text from large language models to solve the problem.
\textbf{Diversity Metrics} 
 Evaluation of the diversity of synthetic data is a key part in ensuring its effectiveness in training. The core diversity metrics can be divided into two major categories: surface-level statistical metrics and metrics based on semantic modeling. Surface-level statistical metrics(\citealp{10.1162/coli_a_00540}) achieve rapid quantification based on text vocabulary and syntactic features. For example, Distinct-n reflects the diversity at the vocabulary and phrase levels by calculating the proportion of unique n-grams; Self-BLEU inversely measures similarity through the degree of n-gram matching between samples. These metrics are computationally efficient, but their evaluation logic that relies on word overlap fails to capture synonymous expressions and semantic equivalence.\\
 In contrast, Semantic modeling metrics are quantified at the semantic level through vector embedding and distribution distance. For instance, models like SimCSE(\citealp{2021arXiv210408821G}) based on contextual embedding identify semantic differences by calculating the cosine similarity of sample vectors; distribution distance metrics like KL divergence and Jensen-Shannon divergence realize global semantic diversity evaluation by measuring the distribution difference between generated data and real data. \\
Taking into account the characteristics of text synthetic data, indirect evaluation methods(\citealp{2024arXiv240418231C,2025arXiv250208512Z}) help verify diversity through downstream task performance: in tasks such as text classification and summarization, the generalization ability of the trained model is used to infer the diversity quality of synthetic data inversely.

\textbf{Deep Verification} With the development of large language models, the concept of deep verification has been proposed in recent years. Its purpose is to address the problem of logical and factual loopholes in the content generated by large language models. \citeauthor{DBLP:conf/acl/DhuliawalaKXRLC24} et al. were the first to propose introducing a verification chain mechanism to reduce hallucinations. The work of \citeauthor{DBLP:conf/emnlp/WengZX0HLSLZ23} et al. also proves that large language models can be competent for reasoning after adding a self-checking mechanism. This leads people to think about how to solve the problem of model hallucination. Subsequently, research on deep verification continued to deepen. \citeauthor{DBLP:conf/acl/00010G00NC25} et al. proposed a multi-agent dynamic verification framework. Audit-of-Understanding (\citealp{abdaljalil2025auditofunderstandingposteriorconstrainedinferencemathematical}) proposed a posterior restricted reasoning framework, starting from the internal reasoning path of the model to test whether the generated content is consistent with the implicit assumptions. These studies constitute the backbone of in-depth verification of general large-scale language models, and promote the evolution of models from usability to verifiability and trustworthiness.


==> Archive/acl/sections-2025dec/rw_event_graph.tex <==
\subsection{Personal Knowledge Graph: Event graph}

\textbf{Core Concepts}

In mobile operation data, there are two levels of event concepts: 

\textbf{Atomic Event (AE)}: Corresponds to one or more mobile operations, serving as the smallest, indivisible event unit.

\textbf{Staged Event (SE)}: Composed of multiple atomic events, collectively forming a larger event with complete semantics.

\textbf{Relation}: Edges in the knowledge graph, including: relationships between events and their corresponding attributes (e.g., between events and persons, events and locations); three types of relationships between events: causal relationship (the consequence of event\_A leads to event\_B), parent-child relationship (an atomic event belongs to a staged event), and coreference relationship (two atomic events refer to the same staged event).

\textbf{Formal Definitions}

\textbf{Operation Sequence}:
\[
\text{OPS} = \{op_1, op_2, \ldots, op_n\}
\]
Each operation \(op_i\) includes the following attributes:
- \(op_i.text\): Operation text

- \(op_i.type\): Operation type (e.g., photo, note, calendar)

- \(op_i.time\): Timestamp

- \(op_i.location\): Location

- \(op_i.person\): Participating person

\textbf{Atomic Event}:
\[
\text{AE} = (\text{trigger\_op}, \text{ops\_list}, \text{semantic\_label}, \text{attributes})
\]
- \(\text{trigger\_op}\): The key operation that triggers the atomic event (usually the first operation)

- \(\text{ops\_list}\): All included operations \(\{op_i, op_{i+1}, \ldots, op_j\}\)

- \(\text{semantic\_label}\): Event type label (e.g., course, meeting, exercise)

- \(\text{attributes} = \{\text{type, time\_range, locations, persons}\}\): Aggregated attributes

\textbf{Staged Event}:
\[
\text{SE} = (\text{trigger\_ae}, \text{ae\_list}, \text{semantic\_label}, \text{properties})
\]
- \(\text{trigger\_ae}\): The first atomic event of the staged event
- \(\text{ae\_list}\): List of included atomic events

- \(\text{semantic\_label}\): Event type label (e.g., course, meeting, exercise)

- \(\text{properties}\): Aggregated attributes of time, location, and participants

\textbf{Event Graph}:
\[
\text{EventGraph} = (V, E)
\]
Where:
- \(V = \{\text{SE}_1, \text{SE}_2, \ldots, \text{SE}_m\}\): Nodes of staged events

- \(E = \{(se_i, se_j, \text{relation\_type}, \text{confidence})\}\): Directed edges, representing relationships between events

\textbf{Multi-level Event Graph Construction Pipeline}

The pipeline for constructing the multi-level event graph is as follows: input of mobile operation sequences → atomic event detection (trigger identification) → atomic event aggregation → atomic event completion (prediction and supplementation of incomplete events via SLM) → staged event recognition → event relation extraction → final knowledge graph output.

\textbf{Atomic Event Aggregation (Based on Cross-document Event Coreference Resolution)}

\textbf{Task Definition}

\textbf{Scenario}: Mobile operation data is often scattered across multiple source documents, and atomic events belonging to the same staged event may be distributed in different documents. Cross-document event coreference resolution aims to identify sets of atomic events from different documents that refer to the same real-world staged event.

\textbf{Input}:
- A list of atomic events \(\text{AEs} = \{ae_1, ae_2, \ldots, ae_k\}\), where each atomic event contains a document identifier \
(\text{ae}_i.doc_id\) (marking which source document the atomic event comes from)

- Document metadata \(\text{Docs} = \{d_1, d_2, \ldots, d_t\}\), where \(d_m\) includes information such as document type (e.g., calendar, photo, note) and time range

\textbf{Output}:
- Coreferential atomic event clusters \(\text{Clusters} = \{C_1, C_2, \ldots, C_m\}\), where each cluster satisfies:
  - Atomic events in the cluster come from at least one document (supporting intra-document and cross-document aggregation)
  
  - All atomic events in the cluster corefer to the same staged event
  
  - Each cluster is associated with a confidence score \(\text{conf}(C_i)\) (indicating the reliability of coreferential relationships within the cluster)

\textbf{Core Issue}: In cross-document scenarios, identify coreferential relationships between atomic events through multi-dimensional feature matching to form semantically consistent candidate clusters of staged events.

\textbf{Overall Process}: Feature representation → cross-document similarity calculation → coreferential pair identification → clustering to generate coreferential clusters.

\textbf{Submodule 1: Atomic Event Feature Representation}

Atomic events are converted into multi-dimensional feature vectors to adapt to cross-document scenarios:
\[
\text{feat}(ae_i) = [\text{sem\_feat}, \text{temp\_feat}, \text{spat\_feat}, \text{part\_feat}, \text{doc\_feat}]
\]

- \textbf{Semantic Features (sem_feat)}:
  - Word vectors of atomic event semantic labels
  - BERT vectors of trigger operation text

- \textbf{Temporal Features (temp_feat)}:
  - Time range encoding: normalized to timestamps
  - Time granularity features: adjusted according to document type (e.g., calendar events are accurate to the minute, photos may be accurate to the second)

- \textbf{Spatial Features (spat_feat)}:
  - Location entity linking vectors: mapping \(\text{ae}_i.locations\) to vector representations of knowledge graph entities
  - Location text features

- \textbf{Participant Features (part_feat)}:
  - Participant entity vectors: embeddings based on names/IDs
  - Participant role features: role labels such as "host" and "attendee" (if available)

- \textbf{Document Features (doc_feat)}:
  - Mobile operation type encoding: \(\text{one-hot}(ae_i.doc_id.type)\) (distinguishing between calendar/photo/note, etc.)
  - Event type encoding: classification results of Task 1

\textbf{Submodule 2: Cross-document Similarity Calculation}

The coreferential similarity of the pairs of atomic events \((ae_i, ae_j)\) (which can be from the same or different documents) is calculated by integrating multiple features:
\[
\text{sim}(ae_i, ae_j) = \omega_1 \cdot \text{sem\_sim} + \omega_2 \cdot \text{temp\_sim} + \omega_3 \cdot \text{spat\_sim} + \omega_4 \cdot \text{part\_sim} + \omega_5 \cdot \text{doc\_sim}
\]

- Weight parameters: can be optimized through grid search
- Sub-similarity calculation: cosine similarity for text vectors; Jaccard similarity or prefix similarity for locations and persons; exponential decay similarity for time

\textbf{Submodule 3: Identification of coreferential pairs}

A binary classification model is built based on similarity to determine whether atomic event pairs are coreferential:
- Input: \(\text{sim}(ae_i, ae_j)\) + feature differences (e.g. time difference, number of location differences, etc.)

- Model: lightweight gradient boosting tree (e.g., XGBoost), with training data labeled coreferential/non-coreferential atomic event pairs

- Output: coreferential probability \(p(ae_i \leftrightarrow ae_j)\); a pair is determined to be coreferential if \(p \geq \theta\) (threshold \(\theta = 0.6\))

\textbf{Submodule 4: Coreferential Cluster Generation}

An undirected graph is constructed based on coreferential pairs, and final clusters are generated through clustering:
- Graph definition: nodes are atomic events, and edge weights are coreferential probabilities \(p(ae_i \leftrightarrow ae_j)\)

- Clustering algorithm: density-based DBSCAN (adapting to clusters of different sizes), where:
  - \(\epsilon\) (neighborhood radius) = 0.5 (coreferential probability threshold)
  
  - \(\text{minPts}\) (minimum number of points) = 2 (at least 2 atomic events form a cluster; clusters of single-atomic-events need separate verification)
  
Cluster confidence calculation:
\[
\text{conf}(C) = \frac{1}{|C|^2} \sum_{ae_i, ae_j \in C} p(ae_i \leftrightarrow ae_j)
\]
(average coreferential probability within the cluster)

\textbf{Evaluation Metrics}

The resolution of Cross-document event coreference adopts standardized evaluation metrics commonly used in academia.

1. \textbf{MUC (Message Understanding Conference)}:
   Measures the ability to detect cluster boundaries by calculating the score based on the number of "correct merges" and "incorrect merges/splits":
   \[
   \text{MUC} = \frac{\text{Number of correct merges}}{\text{Number of correct merges} + \text{Number of incorrect merges} + \text{Number of incorrect splits}}
   \]

2. \textbf{CEAF (Constrained Entity-Aligned F-Measure)}:
   Aligns predicted clusters with real clusters through optimal bipartite matching and calculates the alignment score:
   \[
   \text{CEAF} = \frac{2 \cdot \sum \text{Overlap of matched pairs}}{\sum |C| + \sum |G|}
   \]

3. \textbf{Average Coreference Accuracy (ACA)}:
   \[
   \text{ACA} = \frac{1}{M} \sum_{C_i \in \text{Clusters}} \text{conf}(C_i) \cdot \text{indicator}(C_i \text{ is a real cluster})
   \]
   (Weighted evaluation combining cluster confidence and real labels)



